Attention-Guided Lidar Segmentation and Odometry Using Image-to-Point Cloud Saliency Transfer

LiDAR odometry estimation and 3D semantic segmentation are crucial for autonomous driving, which has achieved remarkable advances recently. However, these tasks are challenging due to the imbalance of points in different semantic categories for 3D semantic segmentation and the influence of dynamic objects for LiDAR odometry estimation, which increases the importance of using representative/salient landmarks as reference points for robust feature learning. To address these challenges, we propose a saliency-guided approach that leverages attention information to improve the performance of LiDAR odometry estimation and semantic segmentation models. Unlike in the image domain, only a few studies have addressed point cloud saliency information due to the lack of annotated training data. To alleviate this, we first present a universal framework to transfer saliency distribution knowledge from color images to point clouds, and use this to construct a pseudo-saliency dataset (i.e. FordSaliency) for point clouds. Then, we adopt point cloud-based backbones to learn saliency distribution from pseudo-saliency labels, which is followed by our proposed SalLiDAR module. SalLiDAR is a saliency-guided 3D semantic segmentation model that integrates saliency information to improve segmentation performance. Finally, we introduce SalLONet, a self-supervised saliency-guided LiDAR odometry network that uses the semantic and saliency predictions of SalLiDAR to achieve better odometry estimation. Our extensive experiments on benchmark datasets demonstrate that the proposed SalLiDAR and SalLONet models achieve state-of-the-art performance against existing methods, highlighting the effectiveness of image-to-LiDAR saliency knowledge transfer. Source code will be available at https://github.com/nevrez/SalLONet.

==> Fig_data_type_sal.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.98\columnwidth]{figs/data_type_comp.pdf}
    \caption{Comparison of different types of point cloud data. 
  (a) Mesh data and mesh-based saliency result from the study \cite{ding2019point}; (b) point cloud of an indoor scene from the dataset of \cite{armeni20163d}; and (c) point cloud of an outdoor scene from SemanticKITTI \cite{behley2019semantickitti} dataset.}
\label{fig:data_type_sal}
\end{figure}

==> Fig_saliency_projection.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\columnwidth]{figs/saliency_projection.pdf}
  \caption{Illustration of point cloud saliency projection from images.}
  \label{fig:saliency_projection}
\end{figure}

==> sallidar_fig_NUMCLASS_comp.tex <==
\begin{figure}[!ht]
\begin{center}
   \includegraphics[width=0.7\linewidth]{fig_NUMCLASS_comp.pdf} 
\end{center}
   \caption{Comparison of different numbers of classes for classification-based saliency modeling.}
\label{fig:NUMCLASS_comp}
\end{figure}

==> sallidar_fig_data_type_comp.tex <==
\begin{figure}[t]
\begin{center}
% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
  \includegraphics[width=\linewidth]{figs/data_type_comp.pdf} 
\end{center}
  \caption{Comparison of different types of point cloud data. 
  (a) Max Planck mesh data (left) 
%   from \url{https://gfx.cs.princeton.edu/proj/sugcon/models/maxplanck.ply} 
  and mesh-based saliency result (right) from study \cite{ding2019point}; (b) point cloud of indoor scene from dataset of \cite{armeni20163d}; point cloud of outdoor scene from semanticKITTI \cite{behley2019semantickitti}.
  }
\label{fig:data_type_comp}
\end{figure}

==> sallidar_fig_saliency_projection.tex <==
\begin{figure*}[t]
\begin{center}
% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.94\linewidth]{figs/sal_projection.pdf} 
\end{center}
   \caption{Framework overview of LiDAR saliency annotation and model training.}
\label{fig:sal_projection}
\end{figure*}

==> sallidar_tab_semkitti_val.tex <==
\begin{table*}[t]
\caption{Results of proposed models and baselines on SemanticKITTI \cite{behley2019semantickitti} validation set. 
Compared with the baseline, the results with \textbf{Bold} represent the model performance is improved. 
% SalLiDAR-I is the model with saliency distribution as attention loss guiding; SalLiDAR-II is the model with saliency distribution as descriptor; SalLiDAR-IIII is the model with saliency distribution as descriptor and attention loss guiding.
}
\centering
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{c c c c c c c c c c c c c c c c c c c c c}
\hline
\textbf{Methods} & \textbf{mIoU} & \rotatebox{90}{car} &  \rotatebox{90}{bicycle} & \rotatebox{90}{motorcycle} & \rotatebox{90}{truck} & \rotatebox{90}{other-vehicle} & \rotatebox{90}{person} & \rotatebox{90}{bicyclist} & \rotatebox{90}{motorcyclist} & \rotatebox{90}{road} & \rotatebox{90}{parking} & \rotatebox{90}{sidewalk} & \rotatebox{90}{other-ground} &
\rotatebox{90}{building} & \rotatebox{90}{fence} & \rotatebox{90}{vegetation} & \rotatebox{90}{trunk} & \rotatebox{90}{terrain} & \rotatebox{90}{pole} & \rotatebox{90}{traffic-sign} \\
\hline
\hline
* RandLA-Net (baseline) & 55.40 & 94.10 & 11.70 & 33.70 & 64.70 & 52.00 & 57.00 & 73.90 & 0.00  & 92.70 & 43.60 & 80.20 & 0.10 & 87.60 & 44.70 & 84.50 & 63.60 & 75.20 & 54.70 & 39.40 \\ 
% \hline
\textbf{RandLA-Net+SalLiDAR-I} & \bf{55.80} & \bf{94.60} & \bf{15.90} & 32.50 & \bf{67.50} & 50.30 & 55.40 & 72.30 & 0.00  & \bf{92.90} & \bf{45.30} & 79.30 & \bf{0.20} & \bf{88.90} & \bf{47.90} & 84.20 & \bf{64.70} & 72.70 & \bf{55.80} & \bf{40.00} \\ 
% \hline
\textbf{RandLA-Net+SalLiDAR-II} & \bf{56.50} & 93.80 & \bf{17.00} & 32.00 & \bf{79.50} & \bf{56.50} & \bf{57.50} & 70.10 & 0.00  & 92.60 & 42.10 & 80.10 & 0.10 & \bf{88.40} & \bf{50.40} & \bf{85.20} & 61.60 & 74.30 & 52.40 & \bf{40.00} \\ 
% \hline
\textbf{RandLA-Net+SalLiDAR-III} & \bf{56.50} & \bf{94.80} & \bf{14.80} & \bf{39.60} & \bf{67.60} & \bf{55.60} & 56.90 & 72.70 & 0.00  & \bf{92.80} & \bf{45.20} & 79.30 & \bf{0.20} & \bf{88.00} & \bf{47.40} & \bf{85.20} & 62.30 & 74.90 & \bf{56.90} & \bf{39.70} \\ 
\hline
$\ddagger$ Cylinder3D (baseline) & 68.82 & 97.41 & 60.53 & 81.17 & 85.94 & 69.50 & 79.62 & 91.98 & 4.60 & 94.15 & 50.47 & 80.85 & 1.64 & 91.72 & 64.17 & 88.37 & 69.98 & 74.51 & 67.29 & 53.77  \\
% \hline
\textbf{Cylinder3D+SalLiDAR-I} & 68.08 & \bf{97.55} & \bf{62.48} & \bf{84.54} & 85.85 & \bf{72.96} & \bf{79.75} & 91.89 & 2.38 & 94.14 & 44.31 & 80.36 & \bf{2.67} & 91.00 & 60.93 & 86.41 & 66.67 & 69.43 & 67.01 & 53.27  \\
% \hline
\textbf{Cylinder3D+SalLiDAR-II} & 67.54 & \bf{97.49} & 60.01 & 80.13 & \bf{86.38} & \bf{70.53} & 78.46 & 90.64 & 1.66 & \bf{94.50} & 45.16 & \bf{81.49} & \bf{1.55} & 90.93 & 60.93 & 86.53 & 68.46 & 70.45 & 60.20 & 51.79  \\
% \hline
\textbf{Cylinder3D+SalLiDAR-III} & 67.87 & \bf{97.43} & 60.21 & \bf{81.91} & \bf{86.35} & \bf{71.03} &79.43 & 91.42 & 2.29 & \bf{94.56} & 45.07 & \bf{81.51} & 1.26 & 91.04 & 61.05 & 86.78 & 68.55 & 71.09 & 66.56 & 52.03  \\
\hline
\hline
\multicolumn{21}{l}{* PyTorch implementation of RandLA-Net~\cite{hu2020randla}, which is available at: {\url{https://github.com/tsunghan-wu/RandLA-Net-pytorch}}.} \\
\multicolumn{21}{l}{$\ddagger$ The results are obtained from the released version of Cylinder3D model \cite{zhu2021cylindrical} from the work in \cite{hou2022point}: {\url{https://github.com/cardwing/Codes-for-PVKD}}.} \\
\end{tabular}
\label{tab_semantickitti_val}
\end{adjustbox}
\end{table*}
